Thresholded Non-Uniform Fourier Frame-Based Reconstruction for Stripmap SAR

Fourier domain methods are fast algorithms for SAR imaging. They typically involve an interpolation in the frequency domain to re-grid non-uniform data so inverse fast Fourier transforms can be performed. In this paper, we apply a frame reconstruction algorithm, extending the non-uniform fast Fourier transform, to stripmap SAR data. Further, we present an improved thresholded frame reconstruction algorithm for robust performance and improved computational efficiency. We demonstrate compelling results on real stripmap SAR data.

==> part4temp.tex <==
\section{Thresholded Frame Theoretic Reconstruction}

NUFFTs, while computationally efficient, are sensitive to the underlying non-uniform sampling pattern, and may manifest as low quality image reconstructions if $\alpha_n$ are not chosen carefully~\cite{viswanathan2010reconstruction}. In this section, we leverage the recent mathematical theory of frame theoretic methods \AG{(FTMs)} which \AG{address these issues} inherent to NUFFTs. However, as we will demonstrate, the FTM still suffers limitations in its choice of $\alpha_n$ that results in lower reconstruction quality. We introduce \textbf{thresholded frame theoretic reconstruction} (tFTR) as a novel, robust method to achieve state-of-the-art performance on real-world SAR data, while not sacrificing computational efficiency. In Section IV we will present extensive experimental results that validate these claims. 

\subsection{Frame Approximation}

\AG{The frame theoretic method (FTM) was proposed in \cite{gelb2014frame}.  The method interprets the non-uniform Fourier data as samples of a Fourier} \emph{frame}.  A frame is a set of vectors that span a vector space but without the linear independence requirement, \AG{and is often viewed as} an overcomplete basis~\cite{christensen2008frames}. This is useful \AG{since real-world data acquisitions often fail to form a basis for a truncated Fourier approximation, yet are still sampled in such a way to form a truncated frame approximation. In particular in \cite{gelb2014frame} it was demonstrated that by interpreting the data as Fourier frame samples, the weights $\alpha_n$ in (\ref{eq:Anu}) could be analytically determined to improve the robustness and quality of the NUFFT, resulting  in the FTM.}

\HELP{Please see my rewrite above.  I have not read \cite{wang2017sparse}, but I do not think it is the what we did in \cite{gelb2014frame}.  I am guessing it is more like what we did in \cite{song2013approximating}.  However, everything you cite below actually comes from \cite{gelb2014frame}.  \cite{song2013approximating} was a precursor to that but really is more like doing a better uniform resampling algorithm.}  

\AG{Before describing how to link Fourier frames to the NUFFT, we first construct a Fourier frame approximation from the non-uniform Fourier samples acquired in applications such as SAR.  This idea, which we will refer to as the {\em frame approximation} (FA)  was considered separately in \cite{song2013approximating,wang2017sparse}.} %but no link was made from the FA to the NUFFT in those investigations.}
%We exposit \sout{this FA algorithm} \AG{the FTM} and how it approximates the radar image. 
Using the notation from Section II, consider the  image $f(\bold{x})$, sampled non-uniform frequencies $\lambda_n$, window function $w$ of the NUFFT, and the uniform grid of frequencies, $\{\bell_m\}_{m = 1}^M$. The frame approximation (FA)  is given as~\cite{song2013approximating}
\beqa\label{eq:Afa}
(f)(\bolx) \approx \sum\limits_{m=1}^M\sum\limits_{n=1}^N b_{m,n}\hat f(\boll_n)e^{2\pi i \bell_m^T\bolx}/w(\bolx),
\eeqa
where the matrix of coefficients $B = [b_{m,n}]$ is defined by $B=\Psi^\dagger$ where $\Psi$ is defined as
\beqa
\Psi = [\inprod{e^{2\pi i \boll_n^T\bolx},e^{2\pi i \bell_m^T\bolx}/w(\bolx)}].
\eeqa

In other words, the coefficients of the FA ($b_{m,n}$) is determined by the pseudo-inverse of the correlation matrix $\Psi$ between the non-uniform sampled frequencies and the uniform grid of frequencies. \AG{It was shown in \cite{song2013approximating} that the convergence of (\ref{eq:Afa}) to the underlying image is completely determined by the properties of the Fourier basis.  That is, (\ref{eq:Afa}) is essentially a partial sum Fourier approximation of $f$.   As was demonstrated in ~\cite{viswanathan2010reconstruction}, this is {\em not} always the case for (\ref{eq:Anu}), which may fail to converge for certain sampling patterns and choices of $\alpha_n$.

Under the assumption that $\hat{w}$ is neglible outside a small window, the difference between the approximations (\ref{eq:Anu}) and (\ref{eq:Afa} can be bounded by ~\cite{gelb2014frame}}
\beqa\label{eq:bound}
\norm{f_{NUFFT}-f_{FA}}_F^2 \leq K\norm{W\Psi D - I}_F^2,
\eeqa
where $W = [\hat w(\bell_m-\boll_n)]$, the matrix of window function values, $K$ is a constant, and $D$ is a diagonal matrix with $D_{nn} = \alpha_n$. The FA algorithm has been shown to perform better than NUFFTs in simulation~\cite{gelb2014frame,song2013approximating}. The main issue with FA is that it is \emph{slow}. While NUFFTs need $\mathcal{O}(N^2\log N)$ calculations~\cite{andersson2012fast}, FA, because of the pseudo-inverse $\Psi^\dagger$, requires $\mathcal{O}(NM^2)$.  \AG{As will be described in what follows, by minimizing the bound in (\ref{eq:bound}), it is possible to improve the accuracy of the NUFFT while still maintaining its computational efficiency.}

\HELP{Somewhere here you have to write that we are going to approximate (\ref{eq:Afa}) with (\ref{eq:Anu}), only with the weights being a matrix.  That's not clear from what is above, and without it, the rest of what follows doesn't really make sense.}

%\subsection{\sout{Our Method: }Threshold Frame Theoretic Reconstruction}
\subsection{Threshold Frame Theoretic Reconstruction}
\HELP{John, what you originally had was misleading.  We already developed the frame theoretic NFFT in \cite{gelb2014frame}.}
\sout{To synergistically combine the benefits of the frame approximation with the computational efficiency of the NUFFT, we introduce our method of thresholded frame theoretic reconstructions (tFTRs).} \AG{In \cite{gelb2014frame} it was observed} that the matrix $D$ in (\ref{eq:bound}) does not necessarily have to be diagonal. Choosing $D$ to be a full matrix, the full pseudo inverse $D = (W \Psi)^\dagger$ returns the frame approximation (FA). However, this method is slow as noted earlier.   \AG{Instead in \cite{gelb2014frame} $D$ was chosen to be a banded matrix, with $r-1$ sub-diagonals.  It was noted that if $r = 2\log_2{N}$ then the algorithm can still be performed with the same efficiency as the regular NUFFT.  There the method was coined {\em frame theoretic NFFT}, and is written as

but we refer to the technique here as the frame theoretic reconstruction (FTR).}

\AG{While defining $D$ as a banded matrix was suitable for the simulated examples in \cite{gelb2014frame}, as will be demonstrated in our numerical results, it is ill-suited for stripmap SAR settings especially in its tolerance to sub-sampled data.}   Hence in this work we define a threshold on the matrix $D$ so that it is bounded in error but has the flexibility to adapt for real data. The intuition is that we want to threshold the values $D_{nm}= R_\uptau((W \Psi)^{\dagger}_{nm})$ where $R_\uptau(x) = x \text{ if } x \geq \tau$ and zero elsewhere. The way $W \Psi$ is structured, such values will lie upon the diagonal given a high enough threshold \cite{gelb2014frame}. This can be interpreted as taking only the most correlated values of the frame approximation coefficients. 


\noindent \textbf{Error Bound:} We now provide error bounds to ensure our thresholding maintains a good approximation for image reconstruction. We will assume that $D$ is invertible for a given threshold\footnote{We find that even if $D$ is not invertible, tFTR still works well in practice.} and let $c$ be the number of nonzero elements contained in this matrix.

The bound in equation \eqref{eq:bound} can be rewritten as:
\beqa\label{eq:rewrite}
\norm{W\Psi D - I}_F^2 = \norm{D}_F^2\norm{W\Psi - D^\dagger}_F^2
\eeqa
This inequality reveals a balancing act: the bound in \eqref{eq:rewrite} is smallest when $D$ is highly \emph{or} lowly populated. That is, if $\uptau$ is chosen to be relatively small, then the error between $\norm{W\Psi - D^\dagger}$ get closer to zero. On the other hand, if $\uptau$ is relatively large, then the norm of $D$ will be small. This can be seen by expanding its Frobenious norm:
\beqa
\norm{D}_F^2 = \sum\limits_{n=1}^N\sum\limits_{m=1}^M R_{\uptau}(D_{nm})^2 \leq (c\uptau)^2
\eeqa
For computational reasons, we desire fewer nonzero entries for $D$ which this bound justifies.

\noindent \textbf{Computational Complexity:} The values of $W\Psi$ are designed to be highest along the diagonal \cite{gelb2014frame,song2013approximating}. Therefore, we can choose $\uptau$ high enough so the $c$ nonzero entries of $D$ are along the diagonal and $R_\uptau$ requires just $c$ operations. Thus, tFTR requires little computational effort for calculating $D$ as opposed to the original FTR which, at its \emph{best}, requires $N$ operations~\cite{gelb2014frame}. That is, $c << N$, which yields tFTR to be faster than FTR. Once $D$ is calculated, then both methods require a straightforward IFFT, requiring $\mathcal{O}(M\log M)$ operations~\cite{andersson2012fast}. 

\begin{algorithm}[t]
\DontPrintSemicolon
\KwIn{
Fourier data: $\{\hat I((\lambda_n^1, \lambda_p^2)\}_{n=1,p=1}^{N,P}$; an uniformly spaced grid of frequencies:
$\{\ell\}_{m=1}^M$, threshold: $\uptau>0$
}
\KwOut{SAR image $I$}
Initialize $\hat I ^ \ast = \boldsymbol{0}$\;;
\For{n = 1:$N$} {
	$\bol{\hat{f}}\gets \hat \{I(\lambda^1_n,\lambda^2_p)\}_{p=1}^{P}$\;
	$W\gets [\hat{w}(\ell_m-\lambda^2_p)]_{m,p}$\;
	$\Psi_{p,m} = [\inprod{\exp(2\pi i \lambda^2_p x),\exp(2\pi i\ell_m x)/w(x)}]_{p,m}$\;
	$D\gets (R_\tau((W\Psi)^\dagger)$\;
	$\hat I^\ast(\lambda^1_n,:)\gets W D\bol{\hat{f}}\oslash w(\bolx)$ for $\bolx=\tfrac{1}{M}[1,\dots,M]^T$
}
$I\gets \text{$2D$\_IFFT}(\hat I^\ast)$\;
\Return{$I$}\;
\caption{Stripmap SAR Imaging with tFTR}
\label{alg:rma}
\end{algorithm}

\subsection{tFTR Algorithm}\label{subsec:discrete}

To implement our thresholded frame theoretic reconstruction, we observe that the 2D radar data can be viewed as a set of $1D$ slices along the azimuthal direction. For this, reconsider our Fourier data as $\{\hat f((\lambda_n^1,\lambda_p^2))\}_{n,p=1}^{N,P}$ with $\lambda_n$ the azmuthal direction. This way, we can focus our efforts on the associated non-uniformly sampled range data $\lambda_p$. The non-uniformity is addressed by calculating $\Psi$, $W$ and then finding $D = R_\tau((W \Psi)^\dagger)$. The key is that only $D$ has to be found for each slice and the non-uniformity is ``corrected'' via the product $W D \bol{\hat f}$ where $\bol{f}$ is the vectorized slice.  Once this and the division of the window function is done for each $\boll_a$, then the entire set is uniformly distributed and can be inverted via a $2D$ IFFT, yielding the image $I$.  The process is detailed in Algorithm~\ref{alg:rma}.  Note that the formula for $\Psi$ is found analytically.
NUFFTs, while computationally efficient, are sensitive to the underlying non-uniform sampling pattern, and may manifest as low quality image reconstructions if $\alpha_n$ are not chosen carefully~\cite{viswanathan2010reconstruction}. In this section, we leverage the recent mathematical theory of frame theoretic methods \AG{(FTMs)} which \AG{address these issues} inherent to NUFFTs. However, as we will demonstrate, the FTM still suffers limitations in its choice of $\alpha_n$ that results in lower reconstruction quality. We introduce \textbf{thresholded frame theoretic reconstruction} (tFTR) as a novel, robust method to achieve state-of-the-art performance on real-world SAR data, while not sacrificing computational efficiency. In Section IV we will present extensive experimental results that validate these claims. 

\subsection{Frame Approximation}

\AG{The frame theoretic method (FTM) was proposed in \cite{gelb2014frame}.  The method interprets the non-uniform Fourier data as samples of a Fourier} \emph{frame}.  A frame is a set of vectors that span a vector space but without the linear independence requirement, \AG{and is often viewed as} an overcomplete basis~\cite{christensen2008frames}. This is useful \AG{since real-world data acquisitions often fail to form a basis for a truncated Fourier approximation, yet are still sampled in such a way to form a truncated frame approximation. In particular in \cite{gelb2014frame} it was demonstrated that by interpreting the data as Fourier frame samples, the weights $\alpha_n$ in (\ref{eq:Anu}) could be analytically determined to improve the robustness and quality of the NUFFT, resulting  in the FTM.}

\HELP{Please see my rewrite above.  I have not read \cite{wang2017sparse}, but I do not think it is the what we did in \cite{gelb2014frame}.  I am guessing it is more like what we did in \cite{song2013approximating}.  However, everything you cite below actually comes from \cite{gelb2014frame}.  \cite{song2013approximating} was a precursor to that but really is more like doing a better uniform resampling algorithm.}  

\AG{Before describing how to link Fourier frames to the NUFFT, we first construct a Fourier frame approximation from the non-uniform Fourier samples acquired in applications such as SAR.  This idea, which we will refer to as the {\em frame approximation} (FA)  was considered separately in \cite{song2013approximating,wang2017sparse}.} %but no link was made from the FA to the NUFFT in those investigations.}
%We exposit \sout{this FA algorithm} \AG{the FTM} and how it approximates the radar image. 
Using the notation from Section II, consider the  image $f(\bold{x})$, sampled non-uniform frequencies $\lambda_n$, window function $w$ of the NUFFT, and the uniform grid of frequencies, $\{\bell_m\}_{m = 1}^M$. The frame approximation (FA)  is given as~\cite{song2013approximating}
\beqa\label{eq:Afa}
(f)(\bolx) \approx \sum\limits_{m=1}^M\sum\limits_{n=1}^N b_{m,n}\hat f(\boll_n)e^{2\pi i \bell_m^T\bolx}/w(\bolx),
\eeqa
where the matrix of coefficients $B = [b_{m,n}]$ is defined by $B=\Psi^\dagger$ where $\Psi$ is defined as
\beqa
\Psi = [\inprod{e^{2\pi i \boll_n^T\bolx},e^{2\pi i \bell_m^T\bolx}/w(\bolx)}].
\eeqa

In other words, the coefficients of the FA ($b_{m,n}$) is determined by the pseudo-inverse of the correlation matrix $\Psi$ between the non-uniform sampled frequencies and the uniform grid of frequencies. \AG{It was shown in \cite{song2013approximating} that the convergence of (\ref{eq:Afa}) to the underlying image is completely determined by the properties of the Fourier basis.  That is, (\ref{eq:Afa}) is essentially a partial sum Fourier approximation of $f$.   As was demonstrated in ~\cite{viswanathan2010reconstruction}, this is {\em not} always the case for (\ref{eq:Anu}), which may fail to converge for certain sampling patterns and choices of $\alpha_n$.

Under the assumption that $\hat{w}$ is neglible outside a small window, the difference between the approximations (\ref{eq:Anu}) and (\ref{eq:Afa} can be bounded by ~\cite{gelb2014frame}}
\beqa\label{eq:bound}
\norm{f_{NUFFT}-f_{FA}}_F^2 \leq K\norm{W\Psi D - I}_F^2,
\eeqa
where $W = [\hat w(\bell_m-\boll_n)]$, the matrix of window function values, $K$ is a constant, and $D$ is a diagonal matrix with $D_{nn} = \alpha_n$. The FA algorithm has been shown to perform better than NUFFTs in simulation~\cite{gelb2014frame,song2013approximating}. The main issue with FA is that it is \emph{slow}. While NUFFTs need $\mathcal{O}(N^2\log N)$ calculations~\cite{andersson2012fast}, FA, because of the pseudo-inverse $\Psi^\dagger$, requires $\mathcal{O}(NM^2)$.  \AG{As will be described in what follows, by minimizing the bound in (\ref{eq:bound}), it is possible to improve the accuracy of the NUFFT while still maintaining its computational efficiency.}

\HELP{Somewhere here you have to write that we are going to approximate (\ref{eq:Afa}) with (\ref{eq:Anu}), only with the weights being a matrix.  That's not clear from what is above, and without it, the rest of what follows doesn't really make sense.}

%\subsection{\sout{Our Method: }Threshold Frame Theoretic Reconstruction}
\subsection{Threshold Frame Theoretic Reconstruction}
\HELP{John, what you originally had was misleading.  We already developed the frame theoretic NFFT in \cite{gelb2014frame}.}
\sout{To synergistically combine the benefits of the frame approximation with the computational efficiency of the NUFFT, we introduce our method of thresholded frame theoretic reconstructions (tFTRs).} \AG{In \cite{gelb2014frame} it was observed} that the matrix $D$ in (\ref{eq:bound}) does not necessarily have to be diagonal. Choosing $D$ to be a full matrix, the full pseudo inverse $D = (W \Psi)^\dagger$ returns the frame approximation (FA). However, this method is slow as noted earlier.   \AG{Instead in \cite{gelb2014frame} $D$ was chosen to be a $2r-1$-banded matrix, with band $r = 2\log_2{N}$, chosen so that the algorithm could still be performed with the same efficiency as the regular NUFFT.  There the method was coined {\em frame theoretic NFFT}, and can be written in matrix vector form as
\beqa\label{eq:FTNFFT}
{\bf f} \approx \sum\limits_{m=1}^M W\Psi D \hat{\bf f}
\eeqa
where $W, \Psi$ and (band limited) $D$ minimize (\ref{eq:bound}.}  \HELP{The above is most likely incorrect so you will have to fix the notation.  In sequel we will refer to (\ref{eq:FTNFFT}) as the frame theoretic reconstruction (FTR).} \HELP{I am not sure why you want to change the name.  I don't particularly like it because somewhere it should be indicated that this is an NUFFT, which is not apparent from the name.  I suggest leaving it as FTNFFT and then using tFTNFFT.}

\AG{While defining $D$ as a banded matrix was suitable for the simulated examples in \cite{gelb2014frame}, as will be demonstrated in our numerical results, it is ill-suited for stripmap SAR settings especially in its tolerance to sub-sampled data.}   Hence in this work we define a threshold on the matrix $D$ so that it is bounded in error but has the flexibility to adapt for real data. The intuition is that we want to threshold the values $D_{nm}= R_\uptau((W \Psi)^{\dagger}_{nm})$ where $R_\uptau(x) = x \text{ if } x \geq \tau$ and zero elsewhere. The way $W \Psi$ is structured, such values will lie upon the diagonal given a high enough threshold \cite{gelb2014frame}. This can be interpreted as taking only the most correlated values of the frame approximation coefficients. 


\noindent \textbf{Error Bound:} We now provide error bounds to ensure our thresholding maintains a good approximation for image reconstruction. We will assume that $D$ is invertible for a given threshold\footnote{We find that even if $D$ is not invertible, tFTR still works well in practice.} and let $c$ be the number of nonzero elements contained in this matrix.

The bound in equation \eqref{eq:bound} can be rewritten as:
\beqa\label{eq:rewrite}
\norm{W\Psi D - I}_F^2 = \norm{D}_F^2\norm{W\Psi - D^\dagger}_F^2
\eeqa
This inequality reveals a balancing act: the bound in \eqref{eq:rewrite} is smallest when $D$ is highly \emph{or} lowly populated. That is, if $\uptau$ is chosen to be relatively small, then the error between $\norm{W\Psi - D^\dagger}$ get closer to zero. On the other hand, if $\uptau$ is relatively large, then the norm of $D$ will be small. This can be seen by expanding its Frobenious norm:
\beqa
\norm{D}_F^2 = \sum\limits_{n=1}^N\sum\limits_{m=1}^M R_{\uptau}(D_{nm})^2 \leq (c\uptau)^2
\eeqa
For computational reasons, we desire fewer nonzero entries for $D$ which this bound justifies.

\noindent \textbf{Computational Complexity:} The values of $W\Psi$ are designed to be highest along the diagonal \cite{gelb2014frame,song2013approximating}. Therefore, we can choose $\uptau$ high enough so the $c$ nonzero entries of $D$ are along the diagonal and $R_\uptau$ requires just $c$ operations. Thus, tFTR requires little computational effort for calculating $D$ as opposed to the original FTR which, at its \emph{best}, requires $N$ operations~\cite{gelb2014frame}. That is, $c << N$, which yields tFTR to be faster than FTR. Once $D$ is calculated, then both methods require a straightforward IFFT, requiring $\mathcal{O}(M\log M)$ operations~\cite{andersson2012fast}. 

\begin{algorithm}[t]
\DontPrintSemicolon
\KwIn{
Fourier data: $\{\hat I((\lambda_n^1, \lambda_p^2)\}_{n=1,p=1}^{N,P}$; an uniformly spaced grid of frequencies:
$\{\ell\}_{m=1}^M$, threshold: $\uptau>0$
}
\KwOut{SAR image $I$}
Initialize $\hat I ^ \ast = \boldsymbol{0}$\;;
\For{n = 1:$N$} {
	$\bol{\hat{f}}\gets \hat \{I(\lambda^1_n,\lambda^2_p)\}_{p=1}^{P}$\;
	$W\gets [\hat{w}(\ell_m-\lambda^2_p)]_{m,p}$\;
	$\Psi_{p,m} = [\inprod{\exp(2\pi i \lambda^2_p x),\exp(2\pi i\ell_m x)/w(x)}]_{p,m}$\;
	$D\gets (R_\tau((W\Psi)^\dagger)$\;
	$\hat I^\ast(\lambda^1_n,:)\gets W D\bol{\hat{f}}\oslash w(\bolx)$ for $\bolx=\tfrac{1}{M}[1,\dots,M]^T$
}
$I\gets \text{$2D$\_IFFT}(\hat I^\ast)$\;
\Return{$I$}\;
\caption{Stripmap SAR Imaging with tFTR}
\label{alg:rma}
\end{algorithm}

\subsection{tFTR Algorithm}\label{subsec:discrete}

To implement our thresholded frame theoretic reconstruction, we observe that the 2D radar data can be viewed as a set of $1D$ slices along the azimuthal direction. For this, reconsider our Fourier data as $\{\hat f((\lambda_n^1,\lambda_p^2))\}_{n,p=1}^{N,P}$ with $\lambda_n$ the azmuthal direction. This way, we can focus our efforts on the associated non-uniformly sampled range data $\lambda_p$. The non-uniformity is addressed by calculating $\Psi$, $W$ and then finding $D = R_\tau((W \Psi)^\dagger)$. The key is that only $D$ has to be found for each slice and the non-uniformity is ``corrected'' via the product $W D \bol{\hat f}$ where $\bol{f}$ is the vectorized slice.  Once this and the division of the window function is done for each $\boll_a$, then the entire set is uniformly distributed and can be inverted via a $2D$ IFFT, yielding the image $I$.  The process is detailed in Algorithm~\ref{alg:rma}.  Note that the formula for $\Psi$ is found analytically.

